PAC Learning to Sample: On Computational Aspects of Language Generation

The success of language models has motivated theoretical work on learning to sample from distributions on discrete domains. A prominent abstraction is the model of language generation in the limit, introduced by Kleinberg and Mullainathan (NeurIPS 2024), in which the algorithm must generate from the target language after some finite but unspecified number of positive examples. While its positive results are surprisingly general, most guarantees are qualitative. In this work, we seek quantitative guarantees on sample and time complexity, inspired by statistical and computational learning theory. To this end, we study a PAC model of language generation, proposed (in a different context) by De, Diakonikolas, and Servedio (SODA 2015), in which a Boolean concept class $C$ over $\{-1,1\}^n$ defines the target languages: given uniformly random positive examples of an unknown concept $f \in C$, the learner must output a sampler whose output distribution (conditioned on the training data) is close in total variation to the uniform distribution over $f^{-1}(1)$. Their work implicitly gives an efficient algorithm for PAC learning to sample $C$, given three primitives for $C$: an online learner, approximate sampling and counting oracles, and an SQ learner. We ask whether these ingredients, in particular online learnability, are necessary. First, we construct a Boolean concept class $C$ for which online learning is cryptographically hard, yet PAC learning to sample is computationally efficient. Then, we develop new algorithms that use offline ERM oracles instead of online learners, together with approximate sampling/counting oracles for intersections of concepts in $C$ and an SQ learner for $C$. We view our results, together with the work of De, Diakonikolas, and Servedio, as a first step towards understanding the computational complexity of language generation.

==> packages.tex <==
\pdfoutput=1
\usepackage[margin=1in]{geometry}
\usepackage[T1]{fontenc}

%\usepackage{newpxtext,newpxmath}

%%%%%% Load math packages 
%\usepackage[tt=false]{libertine}
\usepackage{mathtools}
\usepackage{amssymb,amsthm}
 % \usepackage{newpxtext}
 % \usepackage[varbb]{newpxmath}
\usepackage[XCharter,vvarbb]{newtx}

\usepackage{physics} 
\usepackage{nicefrac}
%\usepackage{lmodern}
 
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{bbm} 
\usepackage{appendix}
\usepackage{caption}
\RequirePackage{subfigure}
\usepackage{float}

%\usepackage{algorithm}
\usepackage{multicol}
\usepackage[framemethod=TikZ]{mdframed}
\mdfsetup{%
backgroundcolor=gray!10, , %royalBlue!20, 
roundcorner=4pt,
linewidth=1pt}
\usepackage[noend]{algpseudocode}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand\hmmax{0}
\newcommand\bmmax{0}


% ==============================================================================
% SECTION: Typography and Color Enhancements. 
% This section includes all packages and commands for enhancing text and color.
%   ==============================================================================


\usepackage[dvipsnames]{xcolor}
\usepackage{color}
\definecolor{niceRed}{RGB}{190,38,38}
\definecolor{niceYellow}{HTML}{f5b400}
\definecolor{blueGrotto}{HTML}{059DC0}
\definecolor{royalBlue}{HTML}{057DCD}
\definecolor{navyBlue}{HTML}{0B579C}
\definecolor{limeGreen}{HTML}{81B622}
\definecolor{nicePurple}{HTML}{9c27b0}
\definecolor{lightRoyalBlue}{HTML}{def2ff}  
\definecolor{gold}{HTML}{ffa300}

\newcommand{\white}[1]{\textcolor{white}{#1}}
\newcommand*{\red}[1]{\textcolor{red}{#1}}
\newcommand*{\blue}[1]{\textcolor{blue}{#1}}
\newcommand*{\gray}[1]{\textcolor{lightgray}{#1}}

% ============ Reference and Bib Setup  ============
\usepackage{hyperref} 
\usepackage[capitalize,nameinlink]{cleveref}

\hypersetup{
  colorlinks = true, 
  urlcolor = {blueGrotto},
  linkcolor = {royalBlue},
  citecolor = {navyBlue}
}
% % 
\usepackage[
  backref=true,
  backend=biber,
  natbib=true,
  style=alphabetic,
  sorting=alphabeticlabel,
  sortcites=true,
  minbibnames=3,
  maxbibnames=999,
  mincitenames=4,
  maxcitenames=4,
  minalphanames=4,
  maxalphanames=4
]{biblatex}

\usepackage{enumitem}


\DeclareSortingTemplate{alphabeticlabel}{
  \sort[final]{%
    \field{labelalpha} % Sort by the alphabetic label (\eg{}, DKL, DLL)
  }
  \sort{%
    \field{year}   % If labels are the same, sort by year
  }
  \sort{%
    \field{title}  % If both label and year are the same, sort by title
  }
}

\AtBeginRefsection{\GenRefcontextData{sorting=ynt}}
\AtEveryCite{\localrefcontext[sorting=ynt]}
\addbibresource{refs.bib}


\usepackage{algpseudocode}

% ============ Comment Management  ============
\usepackage{color-edits}
%\usepackage[suppress]{color-edits}

\addauthor[Shuchen]{sl}{blue}
\addauthor[Alkis]{ak}{niceRed}


 
\usepackage{tikz}
%\pgfplotsset{compat=1.18} 
\usepackage{bm}

%%%%%%%%%%%% Theorem numbering and cleveref macros 
\theoremstyle{plain} %%%%%% Theorem style 
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{claim}[theorem]{Claim}

%%%%%% Separate numbering scheme 
\newtheorem{assumption}{Assumption}
\newtheorem{infassumption}{Informal Assumption}
\newtheorem{inftheorem}{Informal Theorem}
\newtheorem{minftheorem}{Main Informal Theorem}
\newtheorem{maintheorem}{Main Theorem}
\newtheorem{definition}{Definition}
\newtheorem{infdefinition}{Informal Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{observation}[theorem]{Observation}

\theoremstyle{definition} %%%%%% Definition style              
\newtheorem{example}{Example}

\theoremstyle{remark} %%%%%% Remark Style 
\newtheorem{problem}{Problem}
\newtheorem{remark}{Remark}
\AfterEndEnvironment{definition}{\noindent\ignorespaces}
\AfterEndEnvironment{infdefinition}{\noindent\ignorespaces}
\AfterEndEnvironment{example}{\noindent\ignorespaces}
\AfterEndEnvironment{assumption}{\noindent\ignorespaces}
\AfterEndEnvironment{lemma}{\noindent\ignorespaces}
\AfterEndEnvironment{theorem}{\noindent\ignorespaces}
\AfterEndEnvironment{proposition}{\noindent\ignorespaces}
\AfterEndEnvironment{fact}{\noindent\ignorespaces}
\AfterEndEnvironment{question}{\noindent\ignorespaces}
\AfterEndEnvironment{corollary}{\noindent\ignorespaces}
\AfterEndEnvironment{model}{\noindent\ignorespaces}
\AfterEndEnvironment{remark}{\noindent\ignorespaces}
\AfterEndEnvironment{proof}{\noindent\ignorespaces}
\AfterEndEnvironment{fact}{\noindent\ignorespaces}
\AfterEndEnvironment{minftheorem}{\noindent\ignorespaces}
\AfterEndEnvironment{inftheorem}{\noindent\ignorespaces}
\AfterEndEnvironment{maintheorem}{\noindent\ignorespaces}
\AfterEndEnvironment{restatable}{\noindent\ignorespaces}
\AfterEndEnvironment{observation}{\noindent\ignorespaces}


\crefname{section}{Section}{Sections}
\crefname{theorem}{Theorem}{Theorems}
\crefname{theorem*}{Theorem}{Theorems}
\crefname{inftheorem}{Informal Theorem}{Informal Theorems}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{definition}{Definition}{Definitions}
\crefname{infdefinition}{Informal Definition}{Informal Definitions}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{construction}{Construction}{Constructions}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{claim}{Claim}{Claims}
\crefname{observation}{Observation}{Observations}
\crefname{proposition}{Proposition}{Propositions}
\crefname{fact}{Fact}{Facts}
\crefname{question}{Question}{Questions}
\crefname{problem}{Problem}{Problems}
\crefname{remark}{Remark}{Remarks}
\crefname{example}{Example}{Examples}
\crefname{equation}{Equation}{Equations}
\crefname{appendix}{Appendix}{Appendices}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{model}{Model}{Models}
\crefname{figure}{Figure}{Figures}
\crefname{condition}{Condition}{Conditions}







% ============ Indenting Post Environments ============
\AfterEndEnvironment{definition}{\noindent\ignorespaces}
\AfterEndEnvironment{infdefinition}{\noindent\ignorespaces}
\AfterEndEnvironment{assumption}{\noindent\ignorespaces}
\AfterEndEnvironment{problem}{\noindent\ignorespaces}
\AfterEndEnvironment{lemma}{\noindent\ignorespaces}
\AfterEndEnvironment{theorem}{\noindent\ignorespaces}
\AfterEndEnvironment{proposition}{\noindent\ignorespaces}
\AfterEndEnvironment{fact}{\noindent\ignorespaces}
\AfterEndEnvironment{question}{\noindent\ignorespaces}
\AfterEndEnvironment{corollary}{\noindent\ignorespaces}
\AfterEndEnvironment{model}{\noindent\ignorespaces}
\AfterEndEnvironment{remark}{\noindent\ignorespaces}
\AfterEndEnvironment{proof}{\noindent\ignorespaces}
\AfterEndEnvironment{fact}{\noindent\ignorespaces}
\AfterEndEnvironment{minftheorem}{\noindent\ignorespaces}
\AfterEndEnvironment{inftheorem}{\noindent\ignorespaces}
\AfterEndEnvironment{maintheorem}{\noindent\ignorespaces}
\AfterEndEnvironment{restatable}{\noindent\ignorespaces}
\AfterEndEnvironment{infassumption}
{\noindent\ignorespaces}
\AfterEndEnvironment{infcorollary}{\noindent\ignorespaces}

% ============ Cleverref Macros ============
\crefname{section}{Section}{Sections}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{problem}{Problem}{Problems}
\crefname{program}{Program}{Progams}
\crefname{definition}{Definition}{Definitions}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{construction}{Construction}{Constructions}
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{claim}{Claim}{Claims}
\crefname{observation}{Observation}{Observations}
\crefname{proposition}{Proposition}{Propositions}
\crefname{fact}{Fact}{Facts}
\crefname{question}{Question}{Questions}
\crefname{problem}{Problem}{Problems}
\crefname{remark}{Remark}{Remarks}
\crefname{example}{Example}{Examples}
\crefname{equation}{Equation}{Equations}
\crefname{appendix}{Section}{Sections}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{model}{Model}{Models}
\crefname{figure}{Figure}{Figures}
\crefname{infassumption}{Informal Assumption}{Informal Assumptions}
\crefname{inftheorem}{Informal Theorem}{Informal Theorems}
\crefname{infdefinition}{Informal Definition}{Informal Definitions}
\crefname{minftheorem}{Main Informal Theorem}{Main Informal Theorems}
\crefname{maintheorem}{Main Theorem}{Main Theorems}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{step}{Step}{Steps}
\crefname{result}{Result}{Results}
\crefname{event}{Event}{Events}
\crefname{none}{}{}


\definecolor{myC}{rgb}{0, 255, 255}
\definecolor{myY}{rgb}{204, 204, 0}
\definecolor{myM}{rgb}{255, 0, 255}
\definecolor{secinhead}{RGB}{249,196,95}
\definecolor{lgray}{gray}{0.8}


\usepackage{appendix}
\crefname{appsec}{Appendix}{Appendices}

\linespread{1.05}


%%%%%%%%%%%% Common Sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}

%%%%%%%%%%%% Events
\newcommand{\evE}{\ensuremath{\mathscr{E}}}
\newcommand{\evF}{\ensuremath{\mathscr{F}}}
\newcommand{\evG}{\ensuremath{\mathscr{G}}}
\newcommand{\evH}{\ensuremath{\mathscr{H}}}

%%%%%%%%%%% Math Macros
\newcommand{\zo}{\ensuremath{\inbrace{0, 1}}}
\newcommand{\oo}{\ensuremath{\inbrace{-1, 1}}}
\newcommand{\IntsTo}[1]{\setb{1, 2, \dotsc, #1}}
\newcommand{\IntsTon}{\IntsTo{n}}
\newcommand{\Ex}{\operatornamewithlimits{\mathbb{E}}}
\newcommand{\E}{\operatornamewithlimits{\mathbb{E}}}
\newcommand{\Exp}{\Ex}
\newcommand{\cov}{\ensuremath{\operatornamewithlimits{\rm Cov}}}
\renewcommand{\var}{\ensuremath{\operatornamewithlimits{\rm Var}}}
\renewcommand{\tr}{\ensuremath{\operatornamewithlimits{\rm Tr}}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\sgn}{\operatornamewithlimits{sgn}}
\newcommand\ind{\mathbb{1}}

\newcommand{\nfrac}[2]{\nicefrac{#1}{#2}}
\newcommand{\sfrac}[2]{{#1/#2}} 
\newcommand{\OPT}{\mathrm{OPT}} 
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon} 

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\renewcommand{\bigcupdot}{\charfusion[\mathop]{\bigcup}{\cdot}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

%%%%% Nice transpose
% http://tex.stackexchange.com/a/217624/100722
\makeatletter
\newcommand*{\tran}{{\mathpalette\@tran{}}}
\newcommand*{\@tran}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}
\makeatother

%%%%%%%%%%% Hat-Symbols
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\hf}{\wh{f}}

\newcommand{\hD}{\wh{D}}
\newcommand{\hF}{\wh{F}}
\newcommand{\hR}{\wh{R}}
\newcommand{\hS}{\wh{S}}
\newcommand{\hW}{\wh{W}}

%%%%%%%%%%% Star-Symbols
\newcommand{\sS}{S^*}

%%%%%%%%%%% Overline-Symbols
\renewcommand{\bar}{\overline}
\newcommand{\oE}{\overline{E}}
\newcommand{\oS}{\overline{S}}

%%%%%%%%%%% Tilde-Symbols
\renewcommand{\tilde}{\widetilde}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\tS}{\wt{S}}
\newcommand{\tT}{\wt{T}}

\def\<{\langle}
\def\>{\rangle}


\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\let\P\relax
\newcommand{\P}{\mathbb{P}}

%%%%%%%%%%% Cal-Symbols
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\customcal}[1]{\euscr{#1}}
\newcommand{\cA}{\customcal{A}}
\newcommand{\cB}{\customcal{B}}
\newcommand{\cC}{\customcal{C}}
\newcommand{\cD}{\customcal{D}}
\newcommand{\cE}{\customcal{E}}
\newcommand{\cF}{\customcal{F}}
\newcommand{\cG}{\customcal{G}}
\newcommand{\cH}{\customcal{H}}
\newcommand{\cI}{\customcal{I}}
\newcommand{\cJ}{\customcal{J}}
\newcommand{\cK}{\customcal{K}}
\newcommand{\cL}{\customcal{L}}
\newcommand{\cM}{\customcal{M}}
\newcommand{\cN}{\customcal{N}}
\newcommand{\cO}{\customcal{O}}
\newcommand{\cP}{\customcal{P}} 
\newcommand{\cQ}{\customcal{Q}} 
\newcommand{\cR}{\customcal{R}} 
\newcommand{\cS}{\customcal{S}}
\newcommand{\cT}{\customcal{T}}
\newcommand{\cU}{\customcal{U}}
\newcommand{\cV}{\customcal{V}}
\newcommand{\cW}{\customcal{W}}
\newcommand{\cX}{\customcal{X}}
\newcommand{\cY}{\customcal{Y}}
\newcommand{\cZ}{\customcal{Z}}


% ============ Fancy fonts ============
\DeclareMathAlphabet{\mathdutchcal}{U}{dutchcal}{m}{n}
\SetMathAlphabet{\mathdutchcal}{bold}{U}{dutchcal}{b}{n}
\DeclareMathAlphabet{\mathdutchbcal}{U}{dutchcal}{b}{n}

% \usepackage{newtxtext}
% \usepackage{newtxmath}

\DeclareMathAlphabet\urwscr{U}{urwchancal}{b}{n}%
\DeclareMathAlphabet\rsfscr{U}{rsfso}{m}{n}
\DeclareMathAlphabet\euscr{U}{eus}{m}{n}
\DeclareFontEncoding{LS2}{}{}
\DeclareFontSubstitution{LS2}{stix}{m}{n}
\DeclareMathAlphabet\stixcal{LS2}{stixcal}{m} {n}



\DeclareMathOperator{\lap}{\mathrm{Lap}}

%%%%%%%%%%% Signature schemes

\newcommand{\Gen}{\textsc{Gen}}
\newcommand{\Sign}{\textsc{Sign}}
\newcommand{\Ver}{\textsc{Vrfy}}
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\sk}{\mathsf{sk}}


